Introducing LoCo, a Logic for Configuration Problems

In this paper we present the core of LoCo, a logic-based high-level representation language for expressing configuration problems. LoCo shall allow to model these problems in an intuitive and declarative way, the dynamic aspects of configuration notwithstanding. Our logic enforces that configurations contain only finitely many components and reasoning can be reduced to the task of model construction.

==> eptcsdata.tex <==
\providecommand{\firstpage}{36}
\providecommand{\publicationstatus}{C. Drescher, I. Lynce and R. Treinen (eds.):\\ Workshop on Logics for Component Configuration (LoCoCo 2011)\\
EPTCS 65, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.65.4}{10.4204/EPTCS.65.4}}

